Memory Consistency and Program Transformations

A memory consistency model specifies the allowed behaviors of shared memory concurrent programs. At the language level, these models are known to have a non-trivial impact on the safety of program optimizations, limiting the ability to rearrange/refactor code without introducing new behaviors. Existing programming language memory models try to address this by permitting more (relaxed/weak) concurrent behaviors but are still unable to allow all the desired optimizations. A core problem is that weaker consistency models may also render optimizations unsafe, a conclusion that goes against the intuition of them allowing more behaviors. This exposes an open problem of the compositional interaction between memory consistency semantics and optimizations: which parts of the semantics correspond to allowing/disallowing which set of optimizations is unclear. In this work, we establish a formal foundation suitable enough to understand this compositional nature, decomposing optimizations into a finite set of elementary effects on program execution traces, over which aspects of safety can be assessed. We use this decomposition to identify a desirable compositional property (complete) that would guarantee the safety of optimizations from one memory model to another. We showcase its practicality by proving such a property between Sequential Consistency (SC) and $SC_{RR}$, the latter allowing independent read-read reordering over $SC$. Our work potentially paves way to a new design methodology of programming-language memory models, one that places emphasis on the optimizations desired to be performed.

==> 1.Base/base_meta_seq_sem.tex <==
\subsection{The Role of Sequential Semantics}
    
        \label{subsec:seq-sem}

        In Sec~\ref{subsec:mem-model}, we mentioned that sequential semantics would be required to derive the possible executions of the program.
        Although safety of a transformation w.r.t. memory model has been reduced to safety of its constituent transformation-effects, precisely which effects constitute a transformation of a program is essential to guarantee its safety.
        Intuition tempts us to claim that a program transformation is guaranteed to be safe w.r.t. a memory model irrespective of the sequential semantics if all its possible constituent effects (derived by our conservative approximate of pre-traces) are safe. 
        Surprisingly, this claim turns out to be incorrect.

        Consider the optimization in Fig~\ref{fig:register-spilling}, where we have two conditional branches having the same conditional expression.
        In a sequential program, the compiler may decide to re-read $x$ again after the first conditional block; thereby possibly allowing the reuse of variable $a$ for other purposes before it is used again (such optimizations are commonly performed as part of \textit{register spilling}).
        In this situation, the current pre-trace generation would give us 4 pre-traces for both abstract programs, thus ensuring every pre-trace of the transformed program having a matching pair in the original.
        If the memory model allows introducing a read event as a transformation-effect, this program transformation is safe by Def~\ref{def:transf-safe}.
        However, we can clearly see that the original program can only have 2 pre-traces; the conditional choice we make for both branch points need to match, as the value of $a$ does not change in between.
        If the program consists of a concurrent write $x = 1$ (and assuming the initial value of $x$ being $0$), then such a transformation would result in a new behavior. 
        There would be 2 unmatched pre-traces in the transformed program, resulting in transformation being unsafe. 
        %Figure required here
        \begin{figure*}[htbp]
            \centering
            \includegraphics[scale=0.6]{1.Base/RegisterSpilling.pdf}
            \caption{We require thread-local semantics to rule out cases where introducing a read ($A6$) could be an unsafe program transformation in a concurrent context.}
            \label{fig:register-spilling}
        \end{figure*}
        To address this, we need thread-local reasoning to keep track of the choice we make for every conditional expression $a$.
        For any further conditionals with same expression $a$, we use the same choice, except for the case whenever $a$ is updated/changed. 
        This can happen either by some local computation modifying the value of $a$, or a value of some shared memory read into $a$. 
        In such a situation, we can reset the choice for $a$ to be random.
        With this addition, for the example in Fig~\ref{fig:register-spilling}, instead of having 4 pre-traces synthesized, we will have just 2 for the original program, whereas 4 for the transformed.       
        \begin{remark}
            The above approach can be implemented using live variable analysis, which is routinely performed by optimizing compilers \cite{MuchCompiler}.
        \end{remark}
  
        It is also possible that our set of pre-traces are overly conservative, like those potentially disallowing optimizations not involving any memory events as part of the syntactic change. 
        For instance, consider Figure~\ref{fig:cond-equiv}, where we have one conditional branch point with the expression $a$.
        But since $a$ is a constant $1$, the compiler can simply decide to change the expression to be $true$, resulting in the branch point to change.
        Now, even though the program has arguably not changed in terms of memory events, such a transformation would instead have effects involving elimination and introduction of memory events.
        The modified branch point will not be considered equivalent to the previous one (Def~\ref{def:pre-trace-cmp}), resulting in more pre-trace pairs being identified as comparable.
        Thus, a memory model disallowing eliminations and/or introductions would deem this unsafe. 
        \begin{figure*}[htbp]
            \centering
            \includegraphics[scale=0.6]{1.Base/ConditionalExpChange.pdf}
            \caption{We require thread-local semantics to identify the conditional branch points for both programs are equivalent, thereby allowing us to consider such a program transformation safe.}
            \label{fig:cond-equiv}
        \end{figure*}
        To address this, we once again require thread-local reasoning to assert both the expressions are equivalent.
        This is something the compiler will be able to assert via data-flow analyses.

        \begin{remark}
            Note that for the purpose of understanding the compositional nature between transformations and consistency models, we do not utilize/require sequential semantics. 
            Our results are independent of the choice of thread-local reasoning adopted to filter out pre-traces.
        \end{remark}
        
%-------------------------------------------------------------------------------------------------------------------------------
